Partial Rank Similarity Minimization Method for Quality MOS Prediction of Unseen Speech Synthesis Systems in Zero-Shot and Semi-supervised setting

This paper introduces a novel objective function for quality mean opinion score (MOS) prediction of unseen speech synthesis systems. The proposed function measures the similarity of relative positions of predicted MOS values, in a mini-batch, rather than the actual MOS values. That is the partial rank similarity is measured (PRS) rather than the individual MOS values as with the L1 loss. Our experiments on out-of-domain speech synthesis systems demonstrate that the PRS outperforms L1 loss in zero-shot and semi-supervised settings, exhibiting stronger correlation with ground truth. These findings highlight the importance of considering rank order, as done by PRS, when training MOS prediction models. We also argue that mean squared error and linear correlation coefficient metrics may be unreliable for evaluating MOS prediction models. In conclusion, PRS-trained models provide a robust framework for evaluating speech quality and offer insights for developing high-quality speech synthesis systems. Code and models are available at github.com/nii-yamagishilab/partial_rank_similarity/

==> sections/algo.tex <==
(i) We construct a histogram with $b$ bins (hyperparameter), each containing a count specified by $\boldsymbol{C} = (c_1, c_2, \ldots, c_b)$. If the resulting distribution is imbalanced, it is prone to over-classify the majority group due to its higher prior probability. To address this issue, (ii) we randomly sample the minimum count, $\min(C)$, of pseudo MOS values from each bin and discard the remaining values. A total number of selected pseudo MOS values is $=b*\min(C)$. This simply ensures a balanced distribution of selected pseudo MOS values. 


\begin{algorithm}
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}
\caption{BApMOS}
\begin{algorithmic}[1]
    \State \textbf{Given} $m$ unlabelled audio samples and their corresponding pseudo MOS values $\hat{\boldsymbol{Y}} = (\hat{y}_1, \hat{y}_2, \ldots, \hat{y}_m)$
    \State Step1: \Function{Hist}{$\hat{\boldsymbol{Y}}, b$}
      
  \end{algorithmic}
\label{alg:alg1}
\end{algorithm}








